Diagnosis and Repair for Synthesis from Signal Temporal Logic Specifications

We address the problem of diagnosing and repairing specifications for hybrid systems formalized in signal temporal logic (STL). Our focus is on the setting of automatic synthesis of controllers in a model predictive control (MPC) framework. We build on recent approaches that reduce the controller synthesis problem to solving one or more mixed integer linear programs (MILPs), where infeasibility of a MILP usually indicates unrealizability of the controller synthesis problem. Given an infeasible STL synthesis problem, we present algorithms that provide feedback on the reasons for unrealizability, and suggestions for making it realizable. Our algorithms are sound and complete, i.e., they provide a correct diagnosis, and always terminate with a non-trivial specification that is feasible using the chosen synthesis method, when such a solution exists. We demonstrate the effectiveness of our approach on the synthesis of controllers for various cyber-physical systems, including an autonomous driving application and an aircraft electric power system.

==> proofThm1.tex <==
Suppose 
$\mathcal{M}$ is the MILP encoding of $\mathcal{P}$ as defined in equation~\eqref{opt:plain-diagnosis}. Let $\varphi'$, and $\mathcal{D}$ be the output of Algorithm~\ref{algo:DiagnosisRepair}, $\P' = (f_d, g_d, x_0, \varphi', J)$, and $\mathcal{M}'$ the MILP encoding of $\mathcal{P}'$. 
We let $\mathcal{D}^* \subseteq \mathcal{D}$ be the set of predicates that are  repaired to obtain $\varphi'$.
 
The procedure in Algorithm~\ref{algo:DiagnosisRepair}, modifies $\mathcal{M}$ as follows. For each constraint associated with a predicate in $\mathcal{D}$ at time $t$, the algorithm adds a slack variable $s_{it}$ to the associated predicate $\mu_i$. Such a transformation leads to a feasible MILP $\mathcal{M}''$.
We define $s_i = \max_{t\in \{1,\cdots,H\}} s_{it}$, and $\mathcal{S}_{\mathcal{D}} = \{ s_i | s_i \neq 0\}$. Then, $\mathcal{D}^*$ is the set of $\mu_i$ such that its corresponding slack variables $s_i \in \mathcal{S}_{\mathcal{D}}$. We observe that $\mathcal{M}'$, $\mathcal{M}''$ are both relaxed versions of $\mathcal{M}$. Moreover, each constraint relaxed in $\mathcal{M}''$ is also relaxed in $\mathcal{M}'$ by a slack variable $s_i\geq s_{it}$ for all $t$ . Then, $\mathcal{M}'$ and subsequently $\mathcal{P}'$ are also feasible. 

We now prove, that the ($\varphi'$, $\mathcal{D}$) satisfy the predicate minimality condition in Problem~\ref{prob:diagnosis-simple}.

We recall that $\varphi'$ is obtained by modifying predicates $\mu_i \in \mathcal{D}$ to a new predicate $\mu_i' = \mu_i - s_i$, where $s_i$ is defined above. 
Let $\varphi''$ be another repaired formula, such that $\varphi''$ is feasible, and let $\mathcal{D}''$ be its corresponding set of repaired predicates.
Recall that by definition of IIS and Algorithm~\ref{algo:DiagnosisRepair}, at least one predicate in $\mathcal{D}$ must be repaired for the problem to become feasible~\ie $\mathcal{D}'' \cap \mathcal{D} \neq \emptyset$.
In addition, $\mathcal{D}$ contains all the predicates responsible for infeasibility, so repairing any predicate outside of $\mathcal{D}$ is redundant.
If $\mathcal{D}''\setminus \mathcal{D} \neq \emptyset$, then we only need to consider the reduced set $\bar{\mathcal{D}} = \mathcal{D}'' \cap \mathcal{D}$ for repair. Then, a predicate repair that relaxes the predicates in $\bar{\mathcal{D}}$, by the same amount in $\varphi''$, and by zero for predicates in $\mathcal{D}\setminus \bar{\mathcal{D}}$ is also effective. 
By equation~\eqref{eq:slack1}, the norm of the slack variables in $\varphi'$ is minimal, thus the solution of Algorithm~\ref{algo:DiagnosisRepair} is minimal.
%
% If $|\mathcal{D}''| > |\mathcal{D}|$, then ${\mathcal{D}}'' \cap \mathcal{D} \neq \emptyset$,~\ie there are predicates in $\varphi''$ which are not in the minimal set, and they do not need to be relaxed.
%Without loss of generality, it is enough to only discuss the case where $|\mathcal{D}''| \leq |\mathcal{D}|$.
%We let ${\bf p}$ be a $k \times 1$ vector such that ${\bf p}[i] = 1$ if and only if $\mu_i$ is present in $\mathcal{D}$, the set of predicates in Algorithm~\ref{algo:DiagnosisRepair}.
 %$\mathcal{D} = \{\mu_i \text{ s.t. } [A]_i = 1\}$ be the set of predicates Algorithm~\ref{algo:DiagnosisRepair} returns, 
%By the definition of IIS $\mathcal{D}$ is a minimal set of predicates that are causing the infeasibility. 
%We define $\mathcal{D}_c = \{\mu_i \text{ s.t. } {\bf p}[i] = 0\}$ as a set of predicates, which are feasible in the MILP. Our solution introduces slack variables ${\mathcal{S}}_D = \{s_i \text{ s.t. } \mu_i \in \mathcal{D}\}$, and minimizes the norm of the slack variables:
%We define a $k \times 1$ vector, ${\bf a}$, such that $[A]_i = 1$ if $\mu_i$ is present in $\mathcal{D}$. 
% $\mathcal{D} = \{\mu_i s.t [A]_i = 1\}$ be the set of predicates Algorithm~\ref{algo:DiagnosisRepair} returns, then by the definition of IIS this is the minimal set of predicates that are causing the infeasibility. We define $\mathcal{D}_c = \{\mu_i s.t [A]_i = 0\}$ as a set of predicates which are feasible in the MILP. Our solution introduces slacks ${\mathcal{s}}_D = \{s_i \text{ s.t. } \mu_i \in \mathcal{D}\}$, to $\{\mu_i \in \mathcal{D}\}$ and minimizes the norm of the slacks.
%\begin{equation}
%\begin{aligned}
%	& s_i =  \underset{t \in \{1, \hdots, H\}}{\text{maximize}} & s_{it}  \\
%	& {\bf p}[i] = 1 & \forall i \in {1, \hdots, m} 
%\end{aligned}
%\end{equation}

%We modify $\mu_i$ to $\mu_i' = \mu_i - s_i$ and $s_{it}$ is the slack introduced in the MILP constraint corresponding to predicate $\mu_i$ at horizon point $t \in {1, \hdots, H}$. If we choose, $\hat{s}_i < s_i$, then there exists time points $t' \in \{ 1, \hdots, H\}$ such that $s_{it'} > \hat{s}_i$ where the problem becomes infeasible.
%we need to add additional slack to make it feasible. Hence, we need $s_i =  \underset{t \in \{1, \hdots, H\}}{\text{maximize}} \: s_{it}$
%Now consider, $\varphi''$, we define ${\bf p}''$ such that ${\bf p}'' = 1$ if and only if $\mu_i \in {\mathcal{D}}''$. If $|{\mathcal{D}}''| \geq |{\mathcal{D}}|$, then ${\mathcal{D}}'' \cap \mathcal{D} \neq \emptyset$, there are predicates in $\varphi''$ which are not in the minimal set... Because of the minimality of $\mathcal{D}$... ,\ie they are already feasible in the original MILP and need not be corrected to introducing slacks.
%Looking at the set $\mathcal{D}$, the slack variables introduced by our procedure is ${\mathcal{S}}_D$ and the slacks introduced to this set in $\varphi''$ is ${\mathcal{S}}_{D''} = \{s_i \text{ s.t. } \mu_i \in \mathcal{D}\}$. By our procedure we have $|{\mathcal{S}}_D| \leq |{\mathcal{S}}_{D''}|$. Hence, our solution is minimal with respect to predicates.

==> pseudoCodes.tex <==
\begin{algorithm}
\caption{\small{{\tt DiagnosisRepair}}}\label{algo:DiagnosisRepair}
\scriptsize
\begin{algorithmic}[1]
\medskip
\Procedure{{\tt DiagnosisRepair}}{$\psi$, $f_d$, $x_0$}
  \vspace{1mm}
  \State {$P \gets$ {\tt CreateSynthesisProblem($\psi$, $f_d$, $x_0$)}}
  \vspace{1mm}
  \State {$M \gets$ {\tt CreateMILP($P$)}}
  \vspace{1mm}
  \State {$u^N \gets$ {\tt SynthesizeController($M$)}}
  \vspace{1mm}
  \If {$u^N \neq \null$}
  	\vspace{1mm}
	\State{{\bf return} {\tt SynthesisSuccessful}}
	\vspace{1mm}
  \Else
  	\vspace{1mm}
	\State {$status \gets 0$, $AC \gets 0$}
	\vspace{1mm}
	\While {$status = 0$}
      \vspace{1mm}
      \State{$M' \gets M$}
	  \vspace{1mm}
	  \State{$AC \gets AC \cup$ {\tt Diagnosis($M'$, $P$)}}
	  \vspace{1mm}
	  \State{($AC'$,$w_{AC'}$) $\gets$ {\tt ModifyingConstraints($AC$)}}
	  \vspace{1mm}
	  \State{($status$, $changes$) $\gets$ {\tt Repair($M'$, $AC'$, $w_{AC'}$)}}
	  \vspace{1mm}
	\EndWhile
	\vspace{1mm}
	\State{{\bf return} {\tt RepairSuccessful}}
	\vspace{1mm}
  \EndIf
  \vspace{1mm}
\EndProcedure 
\medskip
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{\small{{\tt Diagnosis}}}\label{algo:Diagnosis}
\scriptsize
\begin{algorithmic}[1]
\medskip
\Procedure{{\tt Diagnosis}}{$M'$, $P$}
  \vspace{1mm}
  \State {$I_p \gets$ {\tt IIS($M'$)}}
  \vspace{1mm}
  \State {$\psi' \gets$ {\tt ExtractPredicates($I_p$)}}
  \vspace{1mm}
  \State {$x_{0}' \gets$ {\tt ExtractInitialConditions($I_p$)}}
  \vspace{1mm}
  \State {$AC \gets$ ($\psi'$, $x_0'$)}\Comment{AC is the set of allowable changes}
  \vspace{1mm}
  \State{{\bf return} $AC$}
  \vspace{1mm}
\EndProcedure 
\medskip
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{\small{{\tt Repair}}}\label{algo:Repair}
\scriptsize
\begin{algorithmic}[1]
\medskip
\Procedure{{\tt Repair}}{$M'$, $AC'$, $w_{AC'}$}
  \vspace{1mm}
  \State {$Obj_{M'} \gets 0$}
  \vspace{1mm}
  \For {$c$ in $AC'$}
  	\vspace{1mm}
	\State{$M'[c] \gets M'[c] + s_c$}
	\vspace{1mm}
	\State {$Obj_{M'} \gets Obj_{M'} + w_{AC'}[c] * norm(s_c, i)$}\Comment{i decides the type of norm}
	\vspace{1mm}
  \EndFor
  \vspace{1mm}
  \State{($status$, $slacks$) $\gets$ {\tt Optimize($M'$)}}
  \vspace{1mm}
  \State{$changes \gets \emptyset$}
  \vspace{1mm}
  \If {$status$ = $1$}
  	\vspace{1mm}
	\State{$changes \gets$ {\tt ExtractFeedback($slacks$)}}
	\vspace{1mm}
  \EndIf
  \vspace{1mm}
  \State{{\bf return} ($status$, $changes$)}
  \vspace{1mm}
\EndProcedure 
\medskip
\end{algorithmic}
\end{algorithm}

==> quadrotor.tex <==
% We now consider the problem of controlling a quadrotor, and providing feedback in the case of failures. 
We assume a quadrotor dynamical model including a $12$-dimensional state based on~\cite{huang2009aerodynamics}. The state variables express the $6$ degrees of freedom for the quadrotor,~\ie position $x, y, z$ and rotation angles $\phi, \theta, \psi$, together with their first derivatives $\dot{x},\dot{y},\dot{z},p,q,r$. Variables $\phi, \theta, \psi$ denote roll, pitch, and yaw of the quadrotor. The system has a $4$-dimensional input, $[u_1\enskip u_2\enskip u_3\enskip u_4]^\top$, where $u_1, u_2$, and $u_3$ are control roll, pitch, and yaw inputs, and $u_4$ is the thrust value applied to the quadrotor. To control the system, we locally linearize the following nonlinear dynamics at every time step:
\small
\begin{equation}
\label{eq:nlindyn}
\openup -1\jot
\begin{aligned}
&f_1= 
	\begin{bmatrix}
		\dot{x} & 
		\dot{y} & \dot{z}
	\end{bmatrix}^\top \\
&f_2 = 
	\begin{bmatrix}
		0 & 
		0& g
			\end{bmatrix}^\top - (1/m) R_1(\dot{x},\dot{y},\dot{z}) 
			\begin{bmatrix}
		0 & 
		0& 0 & u_4
			\end{bmatrix}^\top \\
			&f_3 = R_2(\dot{x},\dot{y},\dot{z}) \begin{bmatrix}p & q & r\end{bmatrix}^\top \\
	&f_4 = I^{-1} 
	\begin{bmatrix}
		u_1 & 
		u_2& u_3
	\end{bmatrix}^\top - R_3(p,q,r) I \begin{bmatrix}p & q & r\end{bmatrix}^\top
\end{aligned}
\end{equation}
\normalsize
%\vspace{-10pt}

Here, $R_1$, $R_2$ and $R_3$ denote rotation matrices relating the body frame and inertial frame, and $I$ denotes the inertial matrix.
Our goal is to synthesize a strategy for the quadrotor to travel from a starting position $(x_0, y_0, z_0) = (0, 0, -0.4)$ to a destination $(x_d, y_d, z_d) = (0, 0, -0.1)$. All the other elements in the state vector and the control input are initialized at zero. We define the following constraints on the quadrotor:
\begin{equation}
\label{eq:quadSTL}
\begin{aligned}
	&\varphi_{\text{h}} = \G_{[0,\infty)}(-1.1 \leq z \leq 0)& \quad \text{\small{Height of Flight Bounds}} &\\
	&\varphi_{\text{roll}}= \G_{[0,\infty)}(|u_{1}| \leq 0.3)&\quad \text{\small{Roll Bounds}} & \\
	&\varphi_{\text{pitch}} = \G_{[0,\infty)}(|u_{2}| \leq 0.3)& \quad \text{\small{Pitch Bounds}} &
		\\
	&\varphi_{\text{thr}} = \G_{[0,\infty)}(0 \leq u_4 \leq 6.5)& \quad \text{\small{Thrust Bounds}} &
\end{aligned}	
\end{equation}
%\dorsa{Mention it is the MPC run}
Our MPC scheme becomes infeasible at time $t = 0.675$~s because $\varphi_{\text{h}}$ and $\varphi_{\text{roll}}$ are both violated. The solver takes less than $0.1$~s to generate the IIS which has 32 constraints, out of which 11 constraints are from the predicates, $\varphi_{\text{h}}$ and $\varphi_{\text{roll}}$, in our specifications. Fig.~\ref{fig:quadInfeas} shows the $3$-dimensional view of the infeasibility. The solid blue line shows the path computed by the MPC framework and taken by the quadrotor. As shown in the figure, the quadrotor travels at the boundary of the allowable $z$-dimension at $t = 0.675$ s.
Our algorithm adds a slack of $1.58$ to $\varphi_{\text{h}}$. We interpret this as the maximum deviation the controller finds for the quadrotor from the boundary while computing the control for the horizon at time $t= 0.675$ s. We modify $\varphi_{\text{h}}$ to:
\begin{equation}
	\varphi_{\text{h}}^{\text{new}} = \G_{[0,\infty)}(-1.1 \leq z \leq 1.58).
\end{equation}
The new specifications makes the MPC problem feasible, and its trajectory is shown  in blue in Fig.~\ref{fig:quadFeas}.
 %The trajectory of the feasible problem is shown in blue in Fig.~\ref{fig:quadFeas}.
\begin{figure}
\begin{subfigure}[b]{0.23\textwidth}
\centering
	\includegraphics[width = \textwidth]{figures/QuadrotorInfeasible-d.pdf}
	\caption{\small{The MPC problem for quadrotor becomes infeasible at time $t=0.675$.}}
	\label{fig:quadInfeas}
\end{subfigure}%
\hspace{10pt}
\begin{subfigure}[b]{0.26\textwidth}
\centering
	\includegraphics[width = \textwidth]{figures/QuadrotorFeasible-d.pdf}
	\caption{\small{Feasible controller trajectory for the quadrotor.}}
	\label{fig:quadFeas}
\end{subfigure}
\caption{\small{Diagnosis and repair of infeasibilities in control of quadrotors, the green rectangle representes the quadrotor.}}
\label{fig:quad}
\end{figure}
%\begin{figure}
%	\includegraphics[scale = 0.5]{figures/QuadrotorInfeasible}
%	\caption{Quadrotor becomes infeasible at time $t=0.675$($3$-dimensional view)}
%	\label{fig:QuadrotorInfeas}
%\end{figure}
%\begin{figure}
%	\includegraphics[scale = 0.5]{figures/QuadrotorInfeasible2}
%	\caption{Quadrotor becomes infeasible at time $t=0.675$($2$-dimensional view)}
%	\label{fig:QuadrotorInfeas2}
%\end{figure}
%\begin{figure}
%	\includegraphics[scale = 0.5]{figures/QuadrotorFeasible}
%	\caption{Feasible quadrotor controller($3$-dimensional view)}
%	\label{fig:QuadrotorFeas}
%\end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "root"
%%% End: 

==> relatedWork.tex <==
\alberto{move this in the introduction!}
The problem of diagnosing and repairing formal requirements has achieved its share of attention in the formal methods community. Ferr{\`{e}}re~\etal performs diagnosis on faulty executions of systems with specifications expressed in LTL and MTL(Metric Temporal Logic)~\cite{traceDiagnostics}.
They identify prime implicants, which are conjunction of literals, as the cause of unsatisfiablity of these properties, and map the failure of a specification to the failure of these prime implicants. Similar definitions of unsatisfiable cores for LTL based on its syntax tree were presented in~\cite{Schuppan09}, where the authors also extend this notion to LTL unrealizability.
Li~\etal consider analyzing counter-strategy graphs for detecting cause of unrealizability while synthesizing human-in-the-loop controllers~\cite{li2014synthesis}.
 Raman~\etal address the problem of categorizing the causes of unrealizability, and how to detect them in high-level robot control specifications. The feedback provided in this work is domain-specific and more easily interpretable by the user~\cite{RamanKG13}.
%While these works concentrate on diagnosing temporal logic specifications, they provide no information on how to repair the specification.

On the repair front, Li~\etal explore a template based approach to automatically generating additional assumptions for unrealizable specifications in a fragment of Linear Temporal Logic (LTL)~\cite{mining}. However, this approach may not always give the designer an assumption which fits their intent. Moreover, the feedback is template based, and can only give feedback of a certain format. The authors insert `holes' or `gaps' in a standard LTL template and iterate over all predicates to fill up the `holes'. Generating feedback is particularly challenging for STL specifications as the causes of unrealizability could be either due to violations of the predicates or violation in the intervals of the temporal operators. The template based approach in~\cite{mining} cannot be easily adopted to STL as we would have to introduce `holes' for both the predicates as well as the bounds on time, which in this case could take an infinite number of possible real values.

Also similar to our approach is that of Nuzzo~\etal, who use complementary slackness and duality theory to generate succinct infeasibility proofs, which are sets of mutually-inconsistent constraints forming the unsatisfiable core of an optimization problem~\cite{smt}.
%Many commercial optimization solvers such as Gurobi and CPLEX have built-in functions to find minimal sets of such conflicting constraints.

%\emph{Signal Temporal Logic(STL)} is a suitable specification language for cyber-physical systems as these systems have hybrid dynamics, and require continuous time specifications~\cite{Maler2004}.
%However,
%%due to the lack of tractable formal verification and validation methods for STL, providing formal guarantees in an exhaustive fashion becomes harder when designing cyber-physical systems.
%the main challenges of reasoning with STL requirements stem from the need of dealing with dense time and real valued signals which can generate undecidable or intractable problems.
%
%Synthesis of controllers from temporal logic specifications is a well-studied topic. Pnueli~\etal show the theoretical complexity of synthesis from \emph{Linear Temporal Logic(LTL)} specifications is a doubly exponential in the size of the specification~\cite{PnueliSynthesis}.
%Piterman~\etal show that a for certain subclass of \emph{LTL} properties, \emph{Generalized Reactivity(1)}, this complexity is quadratic in the size of the state space~\cite{piterman2006synthesis}.
%Recently, Raman~\etal introduced a novel method for synthesizing controllers for hybrid systems whose requirements are specified in STL~\cite{Raman14}.
%The authors encode the system dynamics and the STL requirements on the system as mixed integer linear constraints on system variables; controller synthesis is then formulated as an optimization problem subject to these constraints. This work has also been extended by using a Counter-Example Guided Inductive Synthesis (CEGIS) scheme to synthesize a controller for cyber-physical systems in an adversarial environments~\cite{Raman15}.
%Here, the properties on the system are represented as {\tt A} $\implies$ {\tt G} where {\tt A} and {\tt G} are a conjunction of STL specifications. {\tt A} is a set of assumptions made on the environment or adversary, while {\tt G} is a set of guarantees the system provides given that the environment behaves as defined by the assumptions {\tt A}.
%
%The problem of diagnosing and repairing formal requirements is also one that has achieved its share of attention in the formal methods community. Ferr{\`{e}}re~\etal performs diagnosis on faulty executions of systems with specifications expressed in LTL and MTL(Metric Temporal Logic)~\cite{traceDiagnostics}.
%They identify prime implicants, which are conjunction of literals, as the cause of unsatisfiablity of these properties, and map the failure of a specification to the failure of these prime implicants. Similar definitions of unsatisfiable cores for LTL based on its syntax tree were presented in~\cite{Schuppan09}, where the authors also extend this notion to LTL unrealizability.
%Li~\etal consider analyzing counter-strategy graphs for detecting cause of unrealizability while synthesizing human-in-the-loop controllers~\cite{li2014synthesis}.
% Raman~\etal address the problem of categorizing the causes of unrealizability, and how to detect them in high-level robot control specifications. The feedback provided in this work is domain-specific and more easily interpretable by the user~\cite{RamanKG13}.
%%While these works concentrate on diagnosing temporal logic specifications, they provide no information on how to repair the specification.
%
%On the repair front, Li~\etal explore a template based approach to automatically generating additional assumptions for unrealizable GR1 specifications~\cite{mining}. However, this approach may not always give the designer an assumption which fits their intent. Moreover, the feedback is template based, and can only give feedback of a certain format. The authors insert `holes' or `gaps' in a standard LTL template and iterate over all predicates to fill up the `holes'. Generating feedback is particularly challenging for STL specifications as the causes of unrealizability could be either due to violations of the predicates or violation in the intervals of the temporal operators. The template based approach in~\cite{mining} cannot be easily adopted to STL as we would have to introduce `holes' for both the predicates as well as the bounds on time, which in this case could take an infinite number of possible real values.
%
%Given an unsatisfiable or unrealizable STL specification for a hybrid system, along with a description of its dynamics as an MILP, we modify the STL specification to make the synthesis problem feasible. Since, the controller synthesis problem can be converted to an optimization problem, we convert the system diagnosis problem into explaining infeasibility of an optimization problem. Similar to our approach is that of Nuzzo~\etal, who use complementary slackness and duality theory to generate succinct infeasibility proofs, which are sets of mutually-inconsistent constraints forming the unsatisfiable core of the optimization problem~\cite{smt}. Many commercial optimization solvers such as Gurobi and CPLEX have built-in functions to find minimal sets of such conflicting constraints.

%Diagnosis of temporal properties


%Repair of temporal properties

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "root"
%%% End:


==> timingFeedback.tex <==
Finding a sequence of \emph{time-interval repairs} is more involved. Given predicates $\mathcal{D}=\{\mu_1, \ldots,\mu_d\}$ and corresponding support intervals $\mathcal{S}=\{\sigma_1,\ldots, \sigma_d\}$ returned by \texttt{Diagnosis}. 
For providing feedback we follow the following procedure,
\begin{itemize}
	\item In Algorithm~\ref{algo:Repair}, line 8 returns the slacks introduced o every predicate in $\mathcal{D}$. We first search for the largest time interval $\sigma'_i \subseteq \sigma_i$ such that the slacks variables $s_{\mu_i,t}$ associated to predicate $\mu_i \in \mathcal{D}$ at time $t$ are $0$. For all other $\mu_i \notin \mathcal{D}$, $\sigma'_i = \sigma_i$.
	\item We re-write all temporal operators in terms of $G$. The re-write $F_{[a,b]} \psi = \neg G_{[a,b]} \neg \psi$ and $\psi_1 U_{[a,b]} \psi_2 = G_{[0, a]}(\psi_1 U \psi_2) \wedge F_{[a,b]} (\psi_2)$.
	\item The parse tree of $\varphi$ has 3 types of nodes, \emph{predicates($\nu$)}, \emph{boolean operators($\kappa$)}, and \emph{timed operators($\Delta) = \{G\}$}. We traverse the parse tree from the leaf nodes to the root node and define $\sigma^*_i$ for each node as:
	\begin{equation}
		\sigma^*_i = 
		\begin{cases}
			 \sigma'_i & i \in \nu \\
			 \underset{j \in C(i)}{\bigcap} \sigma^*_i & i \in \{\kappa \cup U_u\}\\
			 \sigma^*_{C(i)} & i \in \Delta 
		\end{cases}
	\end{equation}  
	where $C(i)$ is the children of node $i$, $U_u$ and $U_t$ are the untimed and timed until operator.   
	 
	\item We define $\tau^*$ as the interval repair for a temporal operator $\Delta_j$ as
\begin{equation}
	\tau^*_j = \sigma^*_j 
\end{equation} 

	  
\end{itemize}

If $\tau^{*}_j$ is empty for any $j$,  no time-interval repair is possible. We provide an example of time interval repair in Section~\ref{sec:nonadv}.
